Single-channel speech enhancement using learnable loss mixup

Generalization remains a major problem in supervised learning of single-channel speech enhancement. In this work, we propose learnable loss mixup (LLM), a simple and effortless training diagram, to improve the generalization of deep learning-based speech enhancement models. Loss mixup, of which learnable loss mixup is a special variant, optimizes a mixture of the loss functions of random sample pairs to train a model on virtual training data constructed from these pairs of samples. In learnable loss mixup, by conditioning on the mixed data, the loss functions are mixed using a non-linear mixing function automatically learned via neural parameterization. Our experimental results on the VCTK benchmark show that learnable loss mixup achieves 3.26 PESQ, outperforming the state-of-the-art.

==> IS2019_paper_kit/LaTeX/IEEEtran/tools/README <==

January 11, 2007


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.
 2. the \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later
 3. the IEEE itemize, enumerate and description list environments
 4. the complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

IEEEtrantools.sty should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
1/2007 V1.2 (V1.7 of IEEEtran.cls) changes:

 1. Several commands and enviroments have depreciated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow use of the
    obsolete forms, but with an warning message to the console during
    compilation:
    \IEEEPARstart
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
 
 2. These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. \normalsizebaselineskip no longer provided. 

 4. New \IEEEPARstart controls:
    \IEEEPARstartHEIGHTTEXT, \IEEEPARstartFONTSTYLE, \IEEEPARstartCAPSTYLE,
    \IEEEPARstartWORDFONTSTYLE, \IEEEPARstartWORDCAPSTYLE,
    \IEEEPARstartHOFFSET, \IEEEPARstartITLCORRECT
    and the (output) length \IEEEPARstartletwidth.

 5. Provide for an optional argument to \bstctlcite to provide a way to
    specify a different aux file. Define \bstctlcite even if it has already
    been defined.

********************************** Files **********************************

README                - This file.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************



==> IS2019_paper_kit/LaTeX/tex/sections/acknowledgements.tex <==
\section{Acknowledgements}

The ISCA Board would like to thank the organizing committees of the past INTERSPEECH conferences for their help and for kindly providing the template files. \\
Note to authors: Authors should not use logos in acknowledgement section; rather authors should acknowledge corporations by naming them only.

==> IS2019_paper_kit/LaTeX/tex/sections/background.tex <==
\section{Problem formulation}



    
% \section{Page layout and style}


% Authors should observe the following rules for page layout. A highly recommended way to meet these requirements is to use a given template (Microsoft Word?? or LaTeX) and check details against the corresponding example PDF file. Given templates, Microsoft Word\textregistered\ or \LaTeX, can be adapted/imported easily in other software such as LibreOffice, Apple Pages, Lua\LaTeX, and Xe\LaTeX, but please be careful to match the layout of the provided PDF example.

% % \subsection{Basic layout features}

% % \begin{itemize}
% % \item Proceedings will be printed in DIN A4 format. Authors must submit their papers in DIN A4 format.
% % \item Two columns are used except for the title section and for large figures that may need a full page width.
% % \item Left and right margin are 20 mm each. 
% % \item Column width is 80 mm. 
% % \item Spacing between columns is 10 mm.
% % \item Top margin is 25 mm (except for the first page which is 30 mm to the title top).
% % \item Bottom margin is 35 mm.
% % \item Text height (without headers and footers) is maximum 235 mm.
% % \item Headers and footers must be left empty.
% % \item Check indentations and spacings by comparing to this example file (in PDF).
% % \end{itemize}

% % % \subsubsection{Headings}

% % % Section headings are centered in boldface with the first word capitalized and the rest of the heading in lower case. Sub- headings appear like major headings, except they start at the left margin in the column. Sub-sub-headings appear like sub-headings, except they are in italics and not boldface. See the examples in this file. No more than 3 levels of headings should be used.

% % % % \subsection{Text font}

% % % % Times or Times Roman font is used for the main text. Font size in the main text must be 9 points, and in the References section 8 points. Other font types may be used if needed for special purposes. It is VERY IMPORTANT that while making the final PDF file, you embed all used fonts! To embed the fonts, you may use the following instructions:
% % % % \begin{enumerate}
% % % % \item For Windows users, the bullzip printer can convert any PDF to have embedded and subsetted fonts.
% % % % \item For Linux/Mac users, you may use \\
% % % %   pdftops file.pdf\\
% % % %   pstopdf -dPDFSETTINGS=/prepress file.pdf
% % % % \end{enumerate}

% % % % \LaTeX users: users should use Adobe Type 1 fonts such as Times or Times Roman. These are used automatically by the INTERSPEECH2019.sty style file. Authors must not use Type 3 (bitmap) fonts.

% % % % % \subsection{Figures}

% % % % % All figures must be centered on the column (or page, if the figure spans both columns). Figure captions should follow each figure and have the format given in \autoref{fig:speech_production}.

% % % % % Figures should be preferably line drawings. If they contain gray levels or colors, they should be checked to print well on a high-quality non-color laser printer.

% % % % % Graphics (i.\,e., illustrations, figures) must not use stipple fill patterns because they will not reproduce properly in Adobe PDF. Please use only SOLID FILL COLORS.

% % % % % Figures which span 2 columns (i.\,e., occupy full page width) must be placed at the top or bottom of the page.

% % % % % % \subsection{Tables}

% % % % % % An example of a table is shown in Table~\ref{tab:example}. The caption text must be above the table.

% \loadtable{tab:example}

% % % % % % % \subsection{Equations}

% % % % % % % Equations should be placed on separate lines and numbered. Examples of equations are given below. Particularly,
% \loadeq{eq:xt}
% where \(f_\omega(t)\) is a special warping function
% % % % % % % % % 
% \loadeq{eq:f-omega}
% % % % % % % % 
% % % % % % % A residue theorem states that
% % % % % % % % 
% % % % % % % \begin{equation}
% % % % % % %   \oint_C F(z)\,\mathrm{d}z = 2 \pi j \sum_k \mathrm{Res}[F(z),p_k]
% % % % % % %   \label{eq3}
% % % % % % % \end{equation}
% % % % % % % % 
% % % % % % % Applying (\ref{eq3}) to (\ref{eq1}), it is straightforward to see that
% % % % % % % % 
% % % % % % % \begin{equation}
% % % % % % %   1 + 1 = \pi
% % % % % % %   \label{eq4}
% % % % % % % \end{equation}

% % % % % % % Finally we have proven the secret theorem of all speech sciences. No more math is needed to show how useful the result is!

% \loadfig{fig:speech-production}

% % % % % % % % \subsection{Information for Word users only}

% % % % % % % % For ease of formatting, please use the styles listed in Table 2. The styles are defined in this template file and are shown in the order in which they would be used when writing a paper. When the heading styles in Table 2 are used, section numbers are no longer required to be typed in because they will be automatically numbered by Word. Similarly, reference items will be automatically numbered by Word when the ``Reference'' style is used.

% % % % % % % % % \begin{table}[t]
% % % % % % % % %   \caption{Main predefined styles in Word}
% % % % % % % % %   \label{tab:word_styles}
% % % % % % % % %   \centering
% % % % % % % % %   \begin{tabular}{ll}
% % % % % % % % %     \toprule
% % % % % % % % %     \textbf{Style Name}      & \textbf{Entities in a Paper}                \\
% % % % % % % % %     \midrule
% % % % % % % % %     Title                    & Title                                       \\
% % % % % % % % %     Author                   & Author name                                 \\
% % % % % % % % %     Affiliation              & Author affiliation                          \\
% % % % % % % % %     Email                    & Email address                               \\
% % % % % % % % %     AbstractHeading          & Abstract section heading                    \\
% % % % % % % % %     Body Text                & First paragraph in abstract                 \\
% % % % % % % % %     Body Text Next           & Following paragraphs in abstract            \\
% % % % % % % % %     Index                    & Index terms                                 \\
% % % % % % % % %     1. Heading 1             & 1\textsuperscript{st} level section heading \\
% % % % % % % % %     1.1 Heading 2            & 2\textsuperscript{nd} level section heading \\
% % % % % % % % %     1.1.1 Heading 3          & 3\textsuperscript{rd} level section heading \\
% % % % % % % % %     Body Text                & First paragraph in section                  \\
% % % % % % % % %     Body Text Next           & Following paragraphs in section             \\
% % % % % % % % %     Figure Caption           & Figure caption                              \\
% % % % % % % % %     Table Caption            & Table caption                               \\
% % % % % % % % %     Equation                 & Equations                                   \\
% % % % % % % % %     \textbullet\ List Bullet & Bulleted lists                              \\\relax
% % % % % % % % %     [1] Reference            & References                                  \\
% % % % % % % % %     \bottomrule
% % % % % % % % %   \end{tabular}
% % % % % % % % % \end{table}

% % % % % % % % If your Word document contains equations, you must not save your Word document from ``.docx'' to ``.doc'' because when doing so, Word will convert all equations to images of unacceptably low resolution.

% % % % % % % % % \subsection{Hyperlinks}

% % % % % % % % % For technical reasons, the proceedings editor will strip all active links from the papers during processing. Hyperlinks can be included in your paper, if written in full, e.\,g.\ ``http://www.foo.com/index.html''. The link text must be all black. 
% % % % % % % % % Please make sure that they present no problems in printing to paper.

% % % % % % % % % % \subsection{Multimedia files}

% % % % % % % % % % The INTERSPEECH organizing committee offers the possibility to submit multimedia files. These files are meant for audio-visual illustrations that cannot be conveyed in text, tables and graphs. Just like you would when including graphics, make sure that you have sufficient author rights to the multimedia materials that you submit for publication. The proceedings media will NOT contain readers or players, so be sure to use widely accepted file formats, such as MPEG, Windows WAVE PCM (.wav) or Windows Media Video (.wmv) using standard codecs.

% % % % % % % % % % Your multimedia files must be submitted in a single ZIP file for each separate paper. Within the ZIP file you can use folders and filenames to help organize the multimedia files. In the ZIP file you should include a TEXT or HTML index file which describes the purpose and significance of each multimedia file. From within the manuscript, refer to a multimedia illustration by its filename. Use short file names without blanks for clarity.

% % % % % % % % % % The ZIP file you submit will be included as-is in the proceedings media and will be linked to your paper in the navigation interface of the proceedings. Causal Productions (the publisher) and the conference committee will not check or change the contents of your ZIP file.

% % % % % % % % % % Users of the proceedings who wish to access your multimedia files will click the link to the ZIP file which will then be opened by the operating system of their computer. Access to the contents of the ZIP file will be governed entirely by the operating system of the user's computer.

% % % % % % % % % % \subsection{Page numbering}

% % % % % % % % % % Final page numbers will be added later to the document electronically. \emph{Don't make any footers or headers!}


% % % % % % % % % % % \subsection{References}

% % % % % % % % % % % The reference format is the standard IEEE one. References should be numbered in order of appearance, for example \cite{Davis80-COP}, \cite{Rabiner89-ATO}, \cite[pp.\ 417--422]{Hastie09-TEO}, and \cite{YourName17-XXX}.

% % % % % % % % % % \subsection{Abstract}

% % % % % % % % % % The total length of the abstract is limited to 200 words. The abstract included in your paper and the one you enter during web-based submission must be identical. Avoid non-ASCII characters or symbols as they may not display correctly in the abstract book.

% % % % % % % % % % \subsection{Author affiliation}

% % % % % % % % % % Please list country names as part of the affiliation for each country.

% % % % % % % % % % \subsection{Number of authors in the author list}

% % % % % % % % % % The maximum number of authors in the author list is twenty. If the number of contributing authors is more than twenty, they should be listed in a footnote or in acknowledgement section, as appropriate.

% \subsection{Submitted files}

% Authors are requested to submit PDF files of their manu??scripts. You can use commercially available tools or for instance http://www.pdfforge.org/products/pdfcreator. The PDF file should comply with the following requirements: (a) there must be no PASSWORD protection on the PDF file at all; (b) all fonts must be embedded; and (c) the file must be text searchable (do CTRL-F and try to find a common word such as ???the???). The proceedings editors (Causal Productions) will contact authors of non-complying files to obtain a replacement. In order not to endanger the preparation of the proceedings, papers for which a replacement is not provided timely will be withdrawn.

==> tex/equations.tex <==
%<*eq:xt> 
\begin{equation}
  x(t) = s(f_\omega(t))
  \label{eq1}
\end{equation}
%</eq:xt>

%<*eq:f-omega>
\begin{equation}
  f_\omega(t) = \frac{1}{2 \pi j} \oint_C 
  \frac{\nu^{-1k} \mathrm{d} \nu}
  {(1-\beta\nu^{-1})(\nu^{-1}-\beta)}
  \label{eq2}
\end{equation}
%</eq:f-omega>

%<*eq:noisymodel>
\begin{equation}
    \noisy = \speech + \noise,
\end{equation}
%</eq:noisymodel>

%<*eq:encoding>
\begin{equation}
    \encoding = \encoder(\noisy).
\end{equation}
%</eq:encoding>

%<*eq:sencoding>
\begin{equation}\label{eq:sencoding}
    % \sencoding = \frac{1}{\sqrt{\encdim}} \stransform \encoding,
    \sencoding = \stransform \encoding,
\end{equation}
%</eq:sencoding>

%<*eq:nencoding>
\begin{equation}\label{eq:nencoding}
    % \nencoding = \frac{1}{\sqrt{\encdim}} \ntransform \encoding.
    \nencoding = \ntransform \encoding.
\end{equation}
%</eq:nencoding>

%<*eq:snencoding>
\begin{equation}\label{eq:snencoding}
    \sencoding = \stransform \encoding \quad\textup{and}\quad \nencoding = \ntransform \encoding.
\end{equation}
%</eq:snencoding>

%<*eq:sdecoding>
\begin{equation}
    \recspeech = \sdecoder(\sencoding),
\end{equation}
%</eq:sdecoding>

%<*eq:ndecoding>
\begin{equation}
    \recnoise = \ndecoder(\nencoding).
\end{equation}
%</eq:ndecoding>


%<*eq:sndecoding>
\begin{equation}
    \recspeech = \sdecoder(\sencoding) \quad\textup{and}\quad \recnoise = \ndecoder(\nencoding).
\end{equation}
%</eq:sndecoding>


%<*eq:principal-angles>
\begin{equation}
    \cos{\pangle{i}} \coloneqq \max_{\vect{u}_i\in\mathcal{U}} \max_{\vect{v}_i\in\mathcal{V}} \frac{\transpose{\vect{u}_i}\vect{v}_i}{\normtwo{\vect{u}_i}\normtwo{\vect{v}_i}},
\end{equation}
%</eq:principal-angles>

%<*eq:normalized-affinity>
\begin{equation}
    \aff{\subspace{U}}{\subspace{V}} \coloneqq \left( \frac{\sum_{i=1}^d \cos^2{\pangle{i}}}{d} \right)^{\frac{1}{2}},
\end{equation}
%</eq:normalized-affinity>

%<*eq:affinity>
\begin{equation}
    \aff{\subspace{U}}{\subspace{V}} \coloneqq \left( \sum_{i=1}^d \cos^2{\pangle{i}} \right)^{\frac{1}{2}},
\end{equation}
%</eq:affinity>

%<*eq:affinity2>
\begin{equation}
    \aff{\subspace{U}}{\subspace{V}} = \normf{\transpose{\mtx{U}}\mtx{V}}.
\end{equation}
%</eq:affinity2>

%<*eq:consistency-loss>
\begin{equation}
    \consistencyloss = \frac{1}{|\trainset|}\sum_\trainset \left( \normtwo{\recspeech - \speech}^2 + \noisereg \normtwo{\recnoise - \noise}^2 \right),
\end{equation}
%</eq:consistency-loss>

%<*eq:affinity-loss>
% \begin{equation}\label{eq:affinity-loss}
%     \affinityloss = \normf{\transpose{\stransform}\ntransform}^2 + \orthreg \left( \normf{\transpose{\stransform}\stransform - \idmtx}^2 + \normf{\transpose{\ntransform}\ntransform - \idmtx}^2\right).
% \end{equation}
\begin{align}\label{eq:affinity-loss}
    \affinityloss &= \normf{\transpose{\stransform}\ntransform}^2 \\ \nonumber
    &\;\;\;+ \orthreg \left( \normf{\transpose{\stransform}\stransform - \idmtx}^2 + \normf{\transpose{\ntransform}\ntransform - \idmtx}^2\right).
\end{align}



%</eq:affinity-loss>

%<*eq:total-loss>
\begin{equation}\label{eq:total-loss}
    \totalloss \;=\; \consistencyloss\left(\encoder, \sdecoder, \ndecoder, \stransform, \ntransform \right) + \affinityreg \affinityloss \left( \stransform, \ntransform \right).
\end{equation}
%</eq:total-loss>


%<*eq:erm>
\begin{equation}\label{eq:erm}
    \min \frac{1}{\nsamples} \sum_{j=1}^\nsamples \loss{}\big(\f{\sample{\noisy}{j}}, \sample{\speech}{j}\big),
\end{equation}
%</eq:erm>


%<*eq:mixup-sample>
\begin{equation}\label{eq:mixup-sample}
    \mixup{\noisy} = \mixupparam \sample{\noisy}{j} + (1 - \mixupparam) \sample{\noisy}{k}
\end{equation}
%</eq:mixup-sample>


%<*eq:loss-mixup-loss>
\begin{equation}\label{eq:loss-mixup-loss}
    \totalloss{LM} = \mixupparam \loss{}\big(\f{\mixup{\noisy}}, \sample{\speech}{j}\big) + (1 - \mixupparam) \loss{}\big(\f{\mixup{\noisy}}, \sample{\speech}{k}\big).
\end{equation}
%</eq:loss-mixup-loss>

%<*eq:learnable-loss-mixup-loss>
\begin{equation}\label{eq:learnable-loss-mixup-loss}
    \totalloss{LLM} = \mixingfunc\left(\mixupparam\right) \loss{}\big(\f{\mixup{\noisy}}, \sample{\speech}{j}\big) + (1 - \mixingfunc\left(\mixupparam\right)) \loss{}\big(\f{\mixup{\noisy}}, \sample{\speech}{k}\big).
\end{equation}
%</eq:learnable-loss-mixup-loss>


%<*eq:label-mixup-loss>
\begin{equation}\label{eq:label-mixup-loss}
    \loss{}\big( \f{\mixup{\noisy}}, \mixupparam \sample{\speech}{j} + (1 - \mixupparam) \sample{\speech}{k} \big),
\end{equation}
%</eq:label-mixup-loss>


%<*eq:embed-mlp>
\begin{equation}\label{eqn:embed_mlp}
    % \rho_{\text{output}}(\lambda) = \text{pow}\biggl(\lambda, C \sigma(\text{MLP}(\embed{\mixup{\noisy}}))\biggl).
    \rho(\mixupparam) = \mixupparam^{C \sigma(\mlp{\embed{\mixup{\noisy}}})}
\end{equation}
%</eq:embed-mlp>

==> tex/figures.tex <==
%<*fig:speech-production>
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{IS2019_paper_kit/LaTeX/figures/figure.pdf}
  \caption{Schematic diagram of speech production.}
  \label{fig:speech_production}
\end{figure}
%</fig:speech-production>

%<*network>
\begin{figure}[t]
  \centering
  \includegraphics[width=0.9\linewidth]{IS2019_paper_kit/LaTeX/figures/se-network.jpg}
  \caption{High-level diagram of our network.}
  \label{fig:network}
\end{figure}
%</network>

%<*affinity>
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{IS2019_paper_kit/LaTeX/figures/subspace-affinity.png}
  \caption{Subspace affinity.}
  \label{fig:affinity}
\end{figure}
%</affinity>


%<*loss>
\begin{figure}[t]
  \centering
  \begin{minipage}{.25\textwidth}
    \centering
    \includegraphics[width=\linewidth]{IS2019_paper_kit/LaTeX/figures/consistency_loss.png}
  \end{minipage}
  \begin{minipage}{.25\textwidth}
    \centering
    \includegraphics[width=\linewidth]{IS2019_paper_kit/LaTeX/figures/aff_loss.png}
  \end{minipage}
  \caption{Losses curves. Left: $\consistencyloss$. Right: $\affinityloss$.}
  \label{fig:loss}
\end{figure}
%</loss>


%<*beta-visualization>
\begin{figure}[b]
\centering
\includegraphics[width=\linewidth]{IS2019_paper_kit/LaTeX/figures/beta_visualization_1.pdf}
\caption{PDFs of $\beta(\alpha,\alpha)$ with different $\alpha$. As $\alpha \rightarrow 0$, $\beta$ approaches a delta function at $0.0$ and $1.0$ (mixup becomes ERM). At $\alpha=1$, $\beta$ becomes a uniform distribution. As $\alpha \rightarrow \infty$, $\beta$ approaches a standard normal distribution.}
% \caption{Difference $\alpha$ leads to dramatically different PDFs of $\beta(\alpha,\alpha)$. As $\alpha \rightarrow 0$, $\beta$ approaches a delta function at $0.0$ and $1.0$ (mixup becomes ERM). At $\alpha=1$, $\beta$ becomes a uniform distribution. As $\alpha \rightarrow \infty$, $\beta$ approaches a standard normal distribution.}
\label{fig:beta_visualization}
\end{figure}
%</beta-visualization>

==> tex/tables.tex <==

%<*encoder-diagram>
\begin{table}
    \caption{Encoder architecture.}
    \label{tab:encoder-diagram}
    \centering
        \begin{tabular}{lllll}
        Type & Kernel & Stride & Output & Activation\\ \toprule
        Input &  &  & \sizethree{16}{256}{1} & \\ 
        \midrule
        Conv2d & \sizetwo{5}{3} & \sizetwo{1}{1} & \sizethree{16}{256}{64}  & LReLU\\
        Conv2d & \sizetwo{3}{3} & \sizetwo{1}{2} & \sizethree{16}{128}{128} & LReLU\\
        Conv2d & \sizetwo{3}{3} & \sizetwo{1}{2} & \sizethree{16}{64}{128}  & LReLU\\
        Conv2d & \sizetwo{3}{3} & \sizetwo{1}{2} & \sizethree{16}{32}{128}  & LReLU\\
        Conv2d & \sizetwo{3}{3} & \sizetwo{1}{2} & \sizethree{16}{16}{128}  & LReLU\\
        Conv2d & \sizetwo{3}{3} & \sizetwo{1}{2} & \sizethree{16}{8}{128}   & LReLU\\
        Conv2d & \sizetwo{3}{3} & \sizetwo{1}{2} & \sizethree{16}{4}{128}   & LReLU\\
        Conv2d & \sizetwo{3}{3} & \sizetwo{1}{2} & \sizethree{16}{2}{128}   & LReLU\\
        Conv2d & \sizetwo{3}{3} & \sizetwo{1}{2} & \sizethree{16}{1}{128}   & LReLU\\
        Conv2d & \sizetwo{1}{3} & \sizetwo{2}{1} & \sizethree{8}{1}{256}    & LReLU\\
        Conv2d & \sizetwo{1}{3} & \sizetwo{2}{1} & \sizethree{4}{1}{256}    & LReLU\\
        Conv2d & \sizetwo{1}{3} & \sizetwo{2}{1} & \sizethree{2}{1}{256}    & LReLU\\
        Conv2d & \sizetwo{1}{1} & \sizetwo{2}{1} & \sizethree{1}{1}{256}    &\\
        % \midrule
        % Flatten & & & 512 &\\
        % \midrule
        % Fc & & & 64 & \text{Linear}\\ 
        \bottomrule
        \end{tabular}
\end{table}
%</encoder-diagram>


%<*encoder-diagram-2>
\begin{table}
    \caption{Encoder architecture.}
    \label{tab:encoder-diagram}
    \centering
        \begin{tabular}{lllll}
        Type & Kernel & Stride & Output & Activation\\ \toprule
        Input &  &  & \sizethree{16}{256}{1} & \\ 
        \midrule
        Conv2d & \sizetwo{5}{3} & \sizetwo{1}{1} & \sizethree{16}{\textcolor{red}{256}}{64}  & LReLU\\
        Conv2d & \sizetwo{3}{3} & \sizetwo{1}{2} & \sizethree{16}{\textcolor{red}{128}}{128} & LReLU\\
        Conv2d & \sizetwo{3}{3} & \sizetwo{1}{2} & \sizethree{16}{\textcolor{red}{64}}{128}  & LReLU\\
        Conv2d & \sizetwo{3}{3} & \sizetwo{1}{2} & \sizethree{16}{\textcolor{red}{32}}{128}  & LReLU\\
        Conv2d & \sizetwo{3}{3} & \sizetwo{1}{2} & \sizethree{16}{\textcolor{red}{16}}{128}  & LReLU\\
        Conv2d & \sizetwo{3}{3} & \sizetwo{1}{2} & \sizethree{16}{\textcolor{red}{8}}{128}   & LReLU\\
        Conv2d & \sizetwo{3}{3} & \sizetwo{1}{2} & \sizethree{16}{\textcolor{red}{4}}{128}   & LReLU\\
        Conv2d & \sizetwo{3}{3} & \sizetwo{1}{2} & \sizethree{16}{\textcolor{red}{2}}{128}   & LReLU\\
        Conv2d & \sizetwo{3}{3} & \sizetwo{1}{2} & \sizethree{16}{\textcolor{red}{1}}{128}   & LReLU\\
        Conv2d & \sizetwo{1}{3} & \sizetwo{2}{1} & \sizethree{\textcolor{red}{8}}{1}{256}    & LReLU\\
        Conv2d & \sizetwo{1}{3} & \sizetwo{2}{1} & \sizethree{\textcolor{red}{4}}{1}{256}    & LReLU\\
        Conv2d & \sizetwo{1}{3} & \sizetwo{2}{1} & \sizethree{\textcolor{red}{2}}{1}{256}    & LReLU\\
        Conv2d & \sizetwo{1}{1} & \sizetwo{2}{1} & \sizethree{\textcolor{red}{1}}{1}{256}    &\\
        % \midrule
        % Flatten & & & 512 &\\
        % \midrule
        % Fc & & & 64 & \text{Linear}\\ 
        \bottomrule
        \end{tabular}
\end{table}
%</encoder-diagram-2>

%<*results-with-SSNR>
\begin{table}[th]
  \caption{Speech enhancement benchmark}
  \label{tab:results}
  \centering
 \begin{tabular}{c c c c c c} 
 \toprule
          & PESQ & CSIG & CBAK & COVL & SSNR\\ [0.5ex]
 \midrule
 Noisy    & 1.97 & 3.35 & 2.44 & 2.63 & 1.68\\
 Wiener   & 2.22 & 3.23 & 2.68 & 2.67 & 5.07\\ 
 SEGAN    & 2.16 & 3.48 & 2.94 & 2.80 & 7.73\\
 WaveNet  & N/A  & 3.62 & 3.23 & 2.98 & N/A\\
 MMSE-GAN & 2.53 & 3.80 & 3.12 & 3.14 & N/A\\
 D+M      & 2.73 & 3.94 & 3.35 & 3.33 & \textbf{9.40}\\
 UNet.    & 2.90 & 4.22 & 3.32 & 3.58 & N/A\\
 Ours     & \textbf{3.043} & \textbf{4.30} & \textbf{3.42} & \textbf{3.69} & 7.35\\[1ex]
 \bottomrule
 \end{tabular}
\end{table}
%</results-with-SSNR>

%<*benchmark-results>
\begin{table}[th]
  \caption{Speech enhancement benchmark}
  \label{tab:benchmark-results}
  \centering
  \tablefontsize
 \begin{tabular}{c c c c c} 
 \toprule
          & PESQ & CSIG & CBAK & COVL\\ [0.5ex]
 \midrule
 Noisy    & 1.97 & 3.35 & 2.44 & 2.63\\
    MMSE-GAN \cite{soni2018time} & 2.53 & 3.80 & 3.12 & 3.14  \\
    D+M \cite{yao2019coarse} & 2.73 & 3.94 & 3.35 & 3.33  \\
    UNet \cite{bulut2020low} & 2.90 & 4.22 & 3.32 & 3.58 \\
    UNet-AM \cite{tran2020} & 3.04 & 4.30 & 3.42 & 3.69 \\
    T-GSA \cite{kim2020t} & 3.06 & 4.18 & 3.59 & 3.62 \\
    DEMUCS \cite{defossez2020real} & 3.07 & 4.31 & 3.40 & 3.63 \\
    RHR-Net \cite{abdulbaqi2020residual} & 3.20 & 4.37 & \textbf{4.02} & 3.82 \\
\textbf{Learnable Loss Mixup} & \textbf{3.26} & \textbf{4.49} & 3.27 & \textbf{3.91}\\[1ex]
 \bottomrule
 \end{tabular}
\end{table}
%</benchmark-results>


%<*ablation-results>
\begin{table}[th]
  \caption{Ablation study on VCTK with standard error calculated over 5 random seeds. LLM1: Learnable Label Mixup. LM: Loss Mixup. LLM2: Learnable Loss Mixup.}
  \label{table:ablation-results}
  \centering
  \tablefontsize
 \begin{tabular}{ccccc} 
 \toprule
          & PESQ & CSIG & CBAK & COVL\\ [0.5ex]
 \midrule
ERM & $3.18\pm0.00$ & $4.47\pm0.00$ & $\textbf{3.52}\pm0.02$ & $3.86\pm0.00$ \\
LLM1 & $3.10\pm0.01$ & $4.44\pm0.00$ & $3.41\pm0.01$ & $3.80\pm0.01$ \\
LM & $3.20\pm0.01$ & $4.48\pm0.00$ & $3.36\pm0.01$ & $3.87\pm0.00$ \\
LLM2 & $\textbf{3.26}\pm0.01$ & $\textbf{4.49}\pm0.00$ & $3.27\pm0.01$ & $\textbf{3.91}\pm0.00$ \\[1ex]
 \bottomrule
 \end{tabular}
\end{table}
%</ablation-results>


%<*mixup-unet>
\begin{table}[t]
    % \vspace{-1cm}
    \caption{UNet Architecture}
    \label{table:unet}
    \begin{center}
        % \resizebox{0.4\textwidth}{!}{%
        \tablefontsize
        \begin{tabular}{l l l m{9em}}
        \toprule
        Type & Kernel & Stride & Output\\ \midrule
        Input &  &  & \sizethree{64}{256}{1} \\ 
        % \midrule
        Conv2d & \sizetwo{7}{7} & \sizetwo{1}{1} & \sizethree{64}{256}{128}  \\
        Conv2d & \sizetwo{5}{5} & \sizetwo{1}{2} & \sizethree{64}{128}{128}  \\
        Conv2d & \sizetwo{5}{5} & \sizetwo{1}{1} & \sizethree{64}{128}{128}  \\
        Conv2d & \sizetwo{5}{5} & \sizetwo{1}{2} & \sizethree{64}{64}{128}  \\
        Conv2d & \sizetwo{5}{5} & \sizetwo{1}{1} & \sizethree{64}{64}{128}  \\
        
        Conv2d & \sizetwo{3}{3} & \sizetwo{1}{2} & \sizethree{64}{32}{128}  \\
        Conv2d & \sizetwo{3}{3} & \sizetwo{1}{1} & \sizethree{64}{32}{128}  \\
        \vspace{1mm}
        $\vdots$ & $\vdots$ & $\vdots$ & (Freq. downsampling) \\
        Conv2d & \sizetwo{3}{3} & \sizetwo{1}{1} & \sizethree{64}{4}{128}  \\
        Conv2d & \sizetwo{3}{3} & \sizetwo{1}{2} & \sizethree{64}{2}{128}  \\
        Conv2d & \sizetwo{3}{2} & \sizetwo{1}{1} & \sizethree{64}{2}{128}  \\
        Conv2d & \sizetwo{3}{2} & \sizetwo{1}{2} & \sizethree{64}{1}{128}  \\
        
        Conv2d & \sizetwo{3}{1} & \sizetwo{1}{1} & \sizethree{64}{1}{128}  \\
        Conv2d & \sizetwo{3}{1} & \sizetwo{2}{1} & \sizethree{32}{1}{256}  \\ \vspace{1mm}
        $\vdots$ & $\vdots$ & $\vdots$ & (Time downsampling) \\
        Conv2d & \sizetwo{3}{1} & \sizetwo{1}{1} & \sizethree{4}{1}{256}  \\
        Conv2d & \sizetwo{3}{1} & \sizetwo{2}{1} & \sizethree{2}{1}{256}  \\
        Conv2d & \sizetwo{2}{1} & \sizetwo{1}{1} & \sizethree{2}{1}{256}  \\
        Conv2d & \sizetwo{2}{1} & \sizetwo{2}{1} & \sizethree{1}{1}{512}  \\
        
        SubpixelConv2d & \sizetwo{1}{1} & \sizetwo{2}{1} & \sizethree{2}{1}{256}\\
        Conv2d & \sizetwo{2}{1} & \sizetwo{1}{1} & \sizethree{2}{1}{256}\\
        SubpixelConv2d & \sizetwo{2}{1} & \sizetwo{2}{1} & \sizethree{4}{1}{256}\\
        Conv2d & \sizetwo{3}{1} & \sizetwo{1}{1} & \sizethree{4}{1}{256}\\
        SubpixelConv2d & \sizetwo{3}{1} & \sizetwo{2}{1} & \sizethree{8}{1}{256}\\
        Conv2d & \sizetwo{3}{1} & \sizetwo{1}{1} & \sizethree{8}{1}{256}\\
        \vspace{1mm}
        $\vdots$ & $\vdots$ & $\vdots$ &  (Time upsampling)\\
        SubpixelConv2d & \sizetwo{3}{1} & \sizetwo{2}{1} & \sizethree{64}{1}{128}\\
        Conv2d & \sizetwo{3}{1} & \sizetwo{1}{1} & \sizethree{64}{1}{128}\\
        SubpixelConv2d & \sizetwo{3}{1} & \sizetwo{1}{2} & \sizethree{64}{2}{128}\\
        Conv2d & \sizetwo{3}{2} & \sizetwo{1}{1} & \sizethree{64}{2}{128}\\
        SubpixelConv2d & \sizetwo{3}{2} & \sizetwo{1}{2} & \sizethree{64}{4}{128}\\
        Conv2d & \sizetwo{3}{3} & \sizetwo{1}{1} & \sizethree{64}{4}{128}\\
        SubpixelConv2d & \sizetwo{3}{3} & \sizetwo{1}{2} & \sizethree{64}{8}{128}\\
        Conv2d & \sizetwo{3}{3} & \sizetwo{1}{1} & \sizethree{64}{8}{128}\\
        \vspace{1mm}
        $\vdots$ & $\vdots$ & $\vdots$ & (Freq. upsampling)\\
        SubpixelConv2d & \sizetwo{3}{3} & \sizetwo{1}{2} & \sizethree{64}{64}{128}\\
        Conv2d & \sizetwo{5}{5} & \sizetwo{1}{1} & \sizethree{64}{64}{128}\\
        SubpixelConv2d & \sizetwo{5}{5} & \sizetwo{1}{2} & \sizethree{64}{128}{128}\\
        Conv2d & \sizetwo{5}{5} & \sizetwo{1}{1} & \sizethree{64}{128}{128}\\
        SubpixelConv2d & \sizetwo{5}{5} & \sizetwo{1}{2} & \sizethree{64}{256}{128}\\
        Conv2d & \sizetwo{7}{7} & \sizetwo{1}{1} & \sizethree{64}{256}{1}\\
        % \midrule
        % Flatten & & & 512 &\\
        % \midrule
        % Fc & & & 64 & \text{Linear}\\ 
        \bottomrule
        \end{tabular}
        % }
    \end{center}
    % \vspace{-0.5cm}
\end{table}
%</mixup-unet>

==> tex/theorems.tex <==
%<*thm:correlation>
\begin{theorem}\label{theorem:correlation}
    Assume $\stransform$ and $\ntransform$ are orthonormal bases of $\ssubspace$ and $\nsubspace$, respectively. The correlation between the nonzero speech and noise embeddings is bounded by the  affinity between $\ssubspace$ and $\nsubspace$:
    \begin{equation}
        |\cos(\sencoding, \nencoding)| \leq \aff{\ssubspace}{\nsubspace}.
    \end{equation}
\end{theorem}
%</thm:correlation>

%<*proof:correlation>
\begin{proof}
    Let $\boldsymbol{W} = \transpose{\stransform}\ntransform$, we have
    \begin{equation}\label{}
        |\cos(\sencoding, \nencoding)| = \frac{| \transpose{\sencoding}\nencoding |}{\normtwo{\sencoding}\normtwo{\nencoding}} = \frac{| \transpose{\encoding}\boldsymbol{W}\encoding |}{\normtwo{\encoding}\normtwo{\encoding}} = \left|\frac{ \transpose{\encoding}\boldsymbol{W}\encoding }{\transpose{\encoding}\encoding}\right|,
    \end{equation}
    where the second equality is due to Eq.~(\ref{eq:snencoding}) and the assumption that $\stransform$ and $\ntransform$ are orthonormal bases of $\ssubspace$ and $\nsubspace$, respectively. Let $\mixupparam_1 \leq \mixupparam_2 \leq ... \leq \mixupparam_d$ be the eigenvalues of the symmetric matrix $\boldsymbol{W}$, the min-max theorem implies that the Reyleigh quotient $\frac{ \transpose{\encoding}\boldsymbol{W}\encoding }{\transpose{\encoding}\encoding}$ is bounded \cite{Horn2012}:
        \begin{equation}\label{eq:min-max}
            \mixupparam_1 \leq \frac{ \transpose{\encoding}\boldsymbol{W}\encoding }{\transpose{\encoding}\encoding} \leq \mixupparam_d.
        \end{equation}
    Therefore,
        \begin{equation}\label{eq:min-max2}
            |\cos(\sencoding, \nencoding)| \leq \max_i |\mixupparam_i|.
        \end{equation}
    As $\boldsymbol{W}$ is symmetric, $\max_i |\mixupparam_i| = \singval{\textup{max}}$, where $\singval{\textup{max}}$ is the largest singular value of $\boldsymbol{W}$. We conclude that
    \begin{equation}
        |\cos(\sencoding, \nencoding)| \leq \singval{\textup{max}} \leq \sqrt{\sum_{i=1}^d \singval{i}^2} = \normf{\boldsymbol{W}} = \aff{\ssubspace}{\nsubspace},
    \end{equation}
    where $\singval{i}$'s are the singular values of $\boldsymbol{W}$.
\end{proof}
%</proof:correlation>


%<*thm:label-v-loss>
\begin{restatable}{theorem}{label_v_loss}
The gradient update for the label mixup loss, defined as
    \loadeq{eq:label-mixup-loss}
is identical to that for the \lossmixup loss $\totalloss{LM}$ in (\ref{eq:loss-mixup-loss}) if and only if the gradient of the loss $\loss{}$ is an affine map of the targets.
\end{restatable}
%</thm:label-v-loss>
% \vspace{-0.6cm}

%<*proof:label-v-loss>
\begin{proof}
% \begin{equation*}
% \begin{split}
 Let $\theta$ be the weight of the network. For all $\mixupparam \in [0,1], \nabla_\theta \loss{}(\f{\mixup{\noisy}}, \mixupparam \sample{\speech}{j} + (1-\mixupparam) \sample{\speech}{k})
= \mixupparam \nabla_\theta\mathcal{L}(\f{\mixup{\noisy}}, \sample{\speech}{j}) + (1-\mixupparam) \nabla_\theta\loss{}(\f{\mixup{\noisy}}, \sample{\speech}{k})
= \nabla_\theta \bigl[ \mixupparam \loss{}(\f{\mixup{\noisy}}, \sample{\speech}{j}) + (1-\mixupparam) \loss{}(\f{\mixup{\noisy}}, \sample{\speech}{k}) \bigr]$ which concludes the proof for the theorem.
% \end{split}
% \end{equation*}
\end{proof}
%</proof:label-v-loss>


%<*corr:mixup-classification>
\begin{corollary}
\label{eqn:mixup_classification}
\Lossmixup (\ref{eq:loss-mixup-loss}) and label mixup (\ref{eq:label-mixup-loss}) are equivalent for the cross-entropy and the mean squared error loss.
\end{corollary}
%</corr:mixup-classification>


%<*thm:representation>
\begin{restatable}{theorem}{representation}
\label{thm:representation}
A mixing function $\phi$ can be represented by some monotonically increasing function $\rho$ that satisfies $\rho(0)=0$:
\begin{equation}\label{eq:representation}
\phi(\lambda) = \frac{\rho(\lambda)}{\rho(\lambda) + \rho(1-\lambda)}.
\end{equation}
\end{restatable}
%</thm:representation>


%<*proof:representation>
\begin{proof}
As $\phi(1) = \frac{\rho(1)}{\rho(1) + \rho(0)} = 1$,
$\phi(1-\lambda) = \frac{\rho(1 - \lambda)}{\rho(\lambda) + \rho(1-\lambda)} = 1 - \phi(\lambda)$, and $\quad \phi(\lambda) = \frac{1}{1 + \frac{\rho(1-\lambda)}{\rho(\lambda)}}$ is monotonically increasing, Eq.~(\ref{eq:representation}) satisfies Definition~\ref{eqn:mixing_fn}. This concludes the proof for the theorem. 
\end{proof}
%</proof:representation>
